Neural Networks in Numerical Analysis and Approximation Theory

In this Master Thesis, we study the approximation capabilities of Neural Networks in the context of numerical resolution of elliptic PDEs and Approximation Theory. First of all, in Chapter 1, we introduce the mathematical definition of Neural Networks and perform some basic estimates on their composition and parallelization. Then, we implement in Chapter 2 the Galerkin method using Neural Network. In particular, we manage to build a Neural Network that approximates the inverse of positive-definite symmetric matrices, which allows to get a Garlerkin numerical solution of elliptic PDEs. Finally, in Chapter 3, we introduce the approximation space of Neural Networks, a space which consists of functions in $L^p$ that are approximated at a certain rate when increasing the number of weights of Neural Networks. We find the relation of this space with the Besov space: the smoother a function is, the faster it can be approximated with Neural Networks when increasing the number of weights.

==> Data/introduccion.tex <==
\newpage
\chapter*{Introducción}
\noindent

En los últimos años hemos sido testigos del auge de las redes neuronales. Aunque sus principales aplicaciones son para la resolución de problemas de clasificación como se resume en \cite{LIU201711}, en este Trabajo de Fin de Máster nos centramos en su uso para resoluciones numéricas de ecuaciones diferenciales parciales (EDPs) y Teoría de Aproximación.

A pesar de la popularidad de las redes neuronales y la cantidad de investigación relacionada, casi todo el conocimiento proviene de la evidencia empírica. Por ejemplo, el artículo que popularizó las \textit{Physics Informed Neural Networks} (PINNs), \cite{raissi2019physics}, fundamenta su uso únicamente con ejemplos de implementación. Como se presenta en el mismo trabajo \cite{raissi2019physics}, la idea es minimizar, entre las redes neuronales, algún funcional que mida el error sobre la ecuación, las condiciones iniciales y de borde para obtener una solución aproximada. Dichos experimentos son un éxito en el sentido de que las soluciones de aproximación se aproximan a las soluciones exactas conocidas para varias EDPs clásicas. Otro ejemplo de esta tendencia es el trabajo que introduce los \textit{transformers}, \cite{46201}, un gran avance, de nuevo basado en resultados experimentales.

El estudio teórico de las Redes Neuronales es un campo emergente con muchas preguntas abiertos. Sin embargo, hay algunos resultados teóricos. Veamos algunos de los principales resultados teóricos:

En cuanto a la teoría de la aproximación, el artículo \cite{cybenko1989approximation} de 1989 muestra la densidad de las redes neuronales en el espacio de funciones continuas con un dominio acotado. En el mismo año, las hipótesis de este resultado se reducen en los artículos \cite{hornik1989multilayer} y cuatro años más tarde en \cite{leshno1993multilayer}. En cuanto a los teoremas de densidad, existen resultados tempranos en espacios de Sobolev de primer orden, véase \cite{abdeljawad2022approximations} o \cite{shen2022approximation}. Siguiendo la misma idea, \cite{guhring2021approximation} muestra que las redes neuronales aproximan todas excepto las derivadas de orden superior de una función sobre un espacio de Sobolev. También, en \cite{gribonval2022approximation} los autores enlazan los espacios de Besov y la velocidad de aproximación de funciones por Redes Neuronales.

En lo que concierne resultados numéricos, el artículo \cite{kutyniok2022theoretical} da Redes Neuronales que aproximan el producto y el inverso de matrices. Con estas Redes Neuronales, los autores muestran la capacidades de aproximación las de Redes Neuronales a soluciones de EDPs elípticas. Los teoremas de densidad del párrafo previo tienen numerosos usos en numérico.

Además, podemos encontrar en la literatura un uso de redes neuronales para problemas inversos y de control. Los artículos \cite{puthawala2022globally} y \cite{furuya2024globally} muestran la proximidad arbitraria de redes neuronales inyectivas y Operadores Neuronales respectivamente. Estos resultados son especialmente relevantes para aproximar soluciones de problemas inversos con redes neuronales o aproximar el resolvedor directamente. En \cite{garcia2023control}, los autores presentan cómo utilizar PINNs en el contexto de problemas de control y realizan algunos experimentos.

En esta Tesis de Máster pretendemos explicar los resultados teóricos previamente expuestos. Para ello, la estructura de la tesis es la siguiente:

En el capítulo \ref{chap: intro NN}, definimos las redes neuronales como una secuencia alternante de funciones afines y de activación. La composición de estas funciones nos da la realización de la red neuronal. Las propiedades de esta familia de funciones se estudian en este Trabajo de Fin de Máster, teniendo en cuenta los numerosos parámetros de una Red Neuronal, a saber, las matrices y vectores asociados y el número de funciones afines, que es necesario seguir. Para ello introducimos la notación de \cite{Elbr_chter_2021} para poder operar redes neuronales obteniendo estimaciones sobre el número de parámetros.

En el capítulo \ref{chap: Mult NN}, nuestro principal objetivo es utilizar el método de Galerkin para demostrar que las redes neuronales pueden resolver numéricamente EDP elípticas, como hace nuestra fuente principal \cite{kutyniok2022theoretical}. El método de Galerkin, como se explica en el libro \cite{Quarteroni2016}, se basa en el truncamiento de una base de Hilbert para dar una solución discreta de una EDP elíptica. El problema principal se transforma entonces en la inversión de una matriz, donde podemos aplicar redes neuronales. Demostramos que las redes neuronales pueden realizar tal tarea con un tamaño razonable y, por consiguiente, mostramos la capacidad de las redes neuronales para resolver numéricamente EDPs.

Terminamos este trabajo en el capítulo \ref{chap: space NN} con un estudio sobre una variante de los espacios de aproximación introducidos en nuestra guía \cite{gribonval2022approximation}. Como afirman muchos teoremas universales de aproximación (resultados de densidad para Redes Neuronales), como el de \cite{leshno1993multilayer}, aumentar el tamaño de una Red Neuronal permite aproximar cualquier función razonable. Esto sugiere trabajar sobre los espacios de funciones aproximadas a un ratio fijo con respecto al tamaño de la Red Neuronal. El estudio culmina relacionando estos espacios y los espacios de Besov: cuanto más suave sea una función, más rápido se aproximará al aumentar el número de pesos. 
